Saliency Map Based Data Augmentation

Data augmentation is a commonly applied technique with two seemingly related advantages. With this method one can increase the size of the training set generating new samples and also increase the invariance of the network against the applied transformations. Unfortunately all images contain both relevant and irrelevant features for classification therefore this invariance has to be class specific. In this paper we will present a new method which uses saliency maps to restrict the invariance of neural networks to certain regions, providing higher test accuracy in classification tasks.

==> section2_saliency_maps.tex <==
The goal of using saliency maps (also referred as sensitivity map or pixel attribution map) is to provide a visual explanation about which regions of the input image contribute to the network's decision.

The first method was introduced by Simonyan et al. \cite{simonyan2013deep}. It based on simple \textbf{gradient backpropagation}. In contrast to the gradient calculation during training, the gradients of the predicted class score $S_c$ in respect to the input image pixels $I$ are also determined:

\begin{equation}
   M(I) = \frac{\partial}{\partial I} S_c
\end{equation}

The dimensions of the resulting saliency map $M$ will be equal to the dimensions of the input image, for an RGB image $M \in \mathbb{R}^{m\times n \times 3}$. In order to visualize $M$, it needs to be converted to a single channel map $\hat{M}$.

In the original paper, the authors took the highest value across each channel in every $ij$ pixel position: 

\begin{equation}
   \hat{M_{ij}} = \max_c(M_{ijc})
\end{equation}

Figure \ref{fig:saliency_example} shows an example of this saliency visualization method.

\begin{figure}[htp]
\subfloat{\includegraphics[width=3.0in]{Figs/saliency_example.png}}
\caption{Saliency visualization using the gradient based method from \cite{simonyan2013deep}. The network predicted the right class, Labrador Retriever with 0.71 confidence.}
\label{fig:saliency_example}
\end{figure}

There are two, very similar methods to gradient backpropagation, \textbf{DeconvNet} \cite{zeiler2014visualizing} and \textbf{guided backpropagation} \cite{springenberg2014striving}.
Both methods starts from the target class activation, and calculate the saliency map by applying the reverse operation of all layers (convolution, pooling, activation), and by backpropagation. 

The only significant difference between these three methods, is how the ReLU activation is handled.

Feature map $f^{l+1}$ activation after ReLU is calculated as follows:

\begin{equation}
   f^{l+1} = \max_c(f^l,0)
\end{equation}

In the backward pass, the following functions are used to calculate the reconstructed layer $R^l$ for the backpropagation \cite{simonyan2013deep}, DeconvNet \cite{zeiler2014visualizing} and guided backpropagation \cite{springenberg2014striving} methods respectively:

\begin{equation}
\begin{aligned}
   R^l &= (f^l>0)*R^{l+1} \\
   R^l &= (R^{l+1}>0)*R^{l+1} \\
   R^l &= (f^l>0)*(R^{l+1}>0)*R^{l+1} \\
\end{aligned}
\end{equation}

\vspace*{20px}

An improvement of the gradient based methods is the \textbf{SmoothGrad} technique \cite{smilkov2017smoothgrad}. The authors state that  the derivative of $S_c$ fluctuates greatly at small scales, gradients are not smooth, and local variations of the derivatives introduce noise in the saliency map.

This noise can be eliminated by applying the following steps:
\begin{itemize}
\item Generate $n$ number of images from the original image by adding Gaussian noise.
\item Calculate the saliency map for each image using gradient backpropagation.
\item Averaging the calculated saliency maps.
\end{itemize}

\vspace*{10px}

\textbf{Grad-CAM} \cite{selvaraju2017grad} that stands for Gradient-weighted Class Activation Mapping is one of the most popular saliency technique.

Grad-CAM has two pathways to calculate the gradients (Figure \ref{fig:gradcam_model}). The first one uses guided-backpropagation \cite{springenberg2014striving} to calculate a saliency map.

In the second path, the gradient of the target class activation is propagated back only until the last convolutional layer. Then, the values of this convolutional layer's feature maps are weighted by the backpropagated gradient. After that an average feature map is generated and only the positive values are kept by applying ReLU activation. This average feature map will be resized to the input image size, and merged with the saliency map from the first pathway.

\begin{figure}[htp]
\subfloat{\includegraphics[width=3.0in]{Figs/gradcam_model.png}}
\caption{Saliency visualization using the gradient based method from \cite{selvaraju2017grad}. Description}
\label{fig:gradcam_model}
\end{figure}

\vspace*{10px}

In our method we wanted to use the simplest, computationally efficient saliency map technique, therefore we applied the backpropagation based method from \cite{simonyan2013deep}.
